Leveraging Adaptive Implicit Representation Mapping for Ultra High-Resolution Image Segmentation

Implicit representation mapping (IRM) can translate image features to any continuous resolution, showcasing its potent capability for ultra-high-resolution image segmentation refinement. Current IRM-based methods for refining ultra-high-resolution image segmentation often rely on CNN-based encoders to extract image features and apply a Shared Implicit Representation Mapping Function (SIRMF) to convert pixel-wise features into segmented results. Hence, these methods exhibit two crucial limitations. Firstly, the CNN-based encoder may not effectively capture long-distance information, resulting in a lack of global semantic information in the pixel-wise features. Secondly, SIRMF is shared across all samples, which limits its ability to generalize and handle diverse inputs. To address these limitations, we propose a novel approach that leverages the newly proposed Adaptive Implicit Representation Mapping (AIRM) for ultra-high-resolution Image Segmentation. Specifically, the proposed method comprises two components: (1) the Affinity Empowered Encoder (AEE), a robust feature extractor that leverages the benefits of the transformer architecture and semantic affinity to model long-distance features effectively, and (2) the Adaptive Implicit Representation Mapping Function (AIRMF), which adaptively translates pixel-wise features without neglecting the global semantic information, allowing for flexible and precise feature translation. We evaluated our method on the commonly used ultra-high-resolution segmentation refinement datasets, i.e., BIG and PASCAL VOC 2012. The extensive experiments demonstrate that our method outperforms competitors by a large margin. The code is provided in supplementary material.

==> Ziyu_Zhao_cvpr2024/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> Ziyu_Zhao_cvpr2024/sec/0_abstract.tex <==
\begin{abstract}
%
%
Implicit representation mapping (IRM) can translate image features to any continuous resolution, showcasing its potent capability for ultra-high-resolution image segmentation refinement. Current IRM-based methods for refining ultra-high-resolution image segmentation often rely on CNN-based encoders to extract image features and apply a Shared Implicit Representation Mapping Function (SIRMF) to convert pixel-wise features into segmented results. Hence, these methods exhibit two crucial limitations. Firstly, the CNN-based encoder may not effectively capture long-distance information, resulting in a lack of global semantic information in the pixel-wise features. Secondly, SIRMF is shared across all samples, which limits its ability to generalize and handle diverse inputs.
%
% typically rely on a Shared Implicit Representation Mapping Function (SIRMF) to translate pixel-wise features into segmented results, overlooking its two critical limitations: (1) inadequate generalization capability to handle diverse inputs and (2) a tendency to overlook global semantic information. These two limitations significantly hinder the performance of existing IRM-based methods.
%
To address these limitations, we propose a novel approach
%in this work 
that leverages the newly proposed \textbf{A}daptive \textbf{I}mplicit \textbf{R}epresentation \textbf{M}apping (\textbf{AIRM}) for ultra-high-resolution Image Segmentation. 
%
Specifically, the proposed method comprises two components: (1) the \textbf{Affinity Empowered Encoder (AEE)}, a robust feature extractor that leverages the benefits of the transformer architecture and semantic affinity to model long-distance features effectively, and (2) the \textbf{Adaptive Implicit Representation Mapping Function (AIRMF)}, which adaptively translates pixel-wise features without neglecting the global semantic information, allowing for flexible and precise feature translation.
%
We evaluated our method on the commonly used ultra-high-resolution segmentation refinement datasets, \ie, BIG and PASCAL VOC 2012. The extensive experiments demonstrate that our method outperforms competitors by a large margin. The code is provided in supplementary material.

\end{abstract}

\begin{figure}[t]
  \includegraphics[width=1.0\linewidth]{images/abs.pdf} 
  % \vspace{1pt}
              \captionsetup{font={small}}
  \caption{(a) The existing IRM-based methods utilize a Shared Implicit Representation Mapping Function (SIRMF) to transform pixel-wise latent codes into segmentation results. (b) In contrast, our Adaptive Implicit Representation Mapping Function (AIRMF) maps the pixel-wise latent codes adaptively, without neglecting global semantic information.
}
  \vspace{-15pt}
  \label{fig:fig1}
\end{figure}

==> Ziyu_Zhao_cvpr2024/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

%As camera and display technologies advance rapidly, image resolutions have reached new heights, with 4K and 6K resolutions becoming commonplace. This development offers unique opportunities for tasks like portrait photo enhancement, industrial defect detection, and medical diagnosis. However, these ultra-high resolution (\textbf{UHR}) images also present significant challenges for traditional image segmentation techniques. Firstly, handling the vast number of input pixels is computationally demanding and strains GPU memory resources. Secondly, many existing methods resort to up-sampling the final predictions through interpolation, often failing to capture intricate details in the output masks.
% With the rapid advancement of camera and display technologies, image resolutions have soared, making 4K and 6K resolutions increasingly common. This progress presents unique opportunities in areas such as portrait photo enhancement, industrial defect detection, and medical diagnosis. Yet, these ultra-high resolution (\textbf{UHR}) images pose significant challenges to conventional image segmentation techniques. First, processing the immense volume of input pixels is computationally intensive and strains GPU memory. Second, many existing methods depend on up-sampling final predictions via interpolation, which frequently fails to capture complex details in the output masks.

% Recent works, such as \cite{cheng2020cascadepsp}, leveraged the refinement network by employing a cascade scheme progressively up-sample intermediate refinement results at various resolution stages until the desired target resolution was attained, which is pretty time-consuming. 


% Work of CRM \cite{shen2022high} drew inspiration from the achievements of LIIF \cite{chen2021learning}, aiming to attain infinite segmentation precision presented at any high resolution through continuous representation generation. 

% While CRM reduces the computational complexity compared to the discrete refinement approach used in CascadePSP, it still processes feature vectors for each pixel through an MLP decoder with multiple linear layers, neglecting global semantic information when determining the final segmentation value for each pixel.

% Besides, previous refinement segmentation techniques exclusively relied on \textbf{CNN}, which can potentially fall short in capturing long-range dependencies due to their limited receptive field and contextual awareness. These limitations can significantly compromise the quality of \textbf{UHR} image segmentation in complex scenes. 

%
%
Image segmentation, the process of partitioning pixels of an input image into distinct regions, has shown notable progress. While prior methods excel in the low-resolution segmentation task \cite{long2015fully,krizhevsky2012imagenet,simonyan2014very,lin2017feature, chen2017deeplab,chen2016attention}, addressing the task of ultra-high-resolution segmentation still poses a persistent challenge due to substantial computational demands.
%

To address the ultra-high-resolution image segmentation problem, \cite{cheng2020cascadepsp} proposes a refinement network with a cascade scheme, where the intermediate refinement outcomes are iteratively upsampled to higher resolutions.
%This method entails iteratively up-sampling intermediate refinement outcomes across various resolution stages, 
%ultimately attaining the target resolution. 
Despite achieving surprising results, this progressive process is quite time-consuming.
%
To improve the computational efficiency and reduce the inference time, CRM \cite{shen2022high} draws inspiration from LIIF \cite{chen2021learning} and uses Implicit Representation Mapping (IRM) to achieve the refinement of ultra-high-resolution image segmentation.
%
While exhibiting promising performance, existing IRM-based methods, \eg, CRM and LIIF, typically rely on a CNN-based encoder to extract image features and a Shared Implicit Representation Mapping Function (SIRMF) to translate the pixel-wise features, 
%
overlooking two critical limitations: (1) the CNN-based encoder may struggle to effectively capture long-distance information, leading to a lack of global semantic information in pixel-wise features. (2) SIRMF is shared across all samples, limiting its generalization capability to handle diverse inputs.
%
As a result, these two limitations significantly impact the performance of current IRM-based methods (see the green circle in \figref{fig:fig1}).
%

To address these limitations, our work begins by conducting comprehensive experiments to examine the impact of receptive fields on IRM. We observe that larger receptive fields significantly enhance the performance of IRM. Additionally, we analyze the weaknesses of the existing SIRMF and find that it lacks the generalization capability to handle diverse inputs. Based on these observations, we introduce a novel approach that \textit{Leveraging Adaptive Implicit Representation Mapping (AIRM) for Ultra High-Resolution Image Segmentation}.
%
The proposed network comprises two components: the Affinity Empowered Encoder (AEE) and the Adaptive Implicit Representation Mapping Function (AIRMF). The AEE, responsible for feature extraction, leverages the advantages of transformer architecture and semantic affinity to model long-distance features effectively. Unlike using shared mapping parameters, AIRMF's parameters are predicted by a separate network based on the entire feature extracted by AEE. This enables AIRMF to adaptively translate pixel-wise features without neglecting global semantic information, allowing for flexible and precise feature translation.
%
As a result, the proposed method can extract pixel-wise features with a significantly larger receptive field and translate them into the segmentation result in an adaptive manner, collaborating with global semantic information.
%
Our main contribution is the following.
\begin{itemize}

    \item We conduct comprehensive experiments to explore the impact of receptive fields on IRM and analyze the limitations of the existing SIRMF. The experimental results demonstrate two key findings: (1) Larger receptive fields significantly enhance the performance of IRM, and (2) the existing SIRMF lacks the generalization capability to handle diverse inputs and tends to overlook the global semantic information.

    \item We introduce a novel approach named \textit{Leveraging Adaptive Implicit Representation Mapping for Ultra-High-Resolution Image Segmentation}, which comprises two components: the Affinity Empowered Encoder (AEE) and the Adaptive Implicit Representation Mapping Function (AIRMF). The proposed method can extract pixel-wise features with a significantly larger receptive field and translate them into the segmentation result in an adaptive manner, collaborating with global semantic information.

    \item The extensive experiment results on multiple ultra-high-resolution segmentation refinement datasets demonstrate that our method outperforms competitors by a large margin.
    

    % \item We propose a novel approach for \textbf{UHR} image segmentation using Adaptive Implicit Representation (AIR). The AIR method allows for flexible and precise mapping of pixel-level features, addressing the issue of traditional methods neglecting global semantic information.
    % %
    % \item We have developed a robust feature extractor (\textbf{Affinity Empowered Encoder}) that combines the advantages of transformer architecture and semantic affinity to model long-distance features effectively. This encoder enhances the accuracy and robustness of feature extraction by learning and utilizing semantic affinity.
    % %
    % \item We propose an \textbf{Adaptive Implicit Mapping Function} for flexible and precise mapping of pixel-level features. This function enables more detailed and individualized feature mapping, thereby improving the accuracy and effectiveness of segmentation.
    
\end{itemize}












%We aim to refine the coarse mask that is already acquired from low-level segmentation. Thus, we have harnessed the strengths of Hypernetwork \cite{article} for the task of \textbf{UHR} image segmentation, which is designed to generate parameters for other models. To be more specific, we propose a hypernetwork to model weights and biases for each linear layer from vanilla MLP. Firstly, the self-attention mechanism in Transformers could model the global feature relations and conquer the aforementioned drawback of convolutional neural networks, thus discovering more integral object regions. In addition, multi-head self-attention in Transformers could capture semantic level affinity, and can thus be used to improve the coarse masks.

% Our goal is to refine the coarse mask obtained from low-level segmentation. To this end, we employ Hypernetwork \cite{article} for \textbf{UHR} image segmentation. Hypernetwork is uniquely designed to generate parameters for other models. Specifically, we propose a hypernetwork to model the weights and biases for each layer in a vanilla MLP. Firstly, the self-attention mechanism in Transformers can model global feature relations, overcoming the limitations of convolutional neural networks. This allows for discovering more integral object regions. Additionally, the multi-head self-attention in Transformers can capture semantic-level affinity, which can be leveraged to enhance the coarse masks.

%Based on the above analysis, we propose a Transformer-based continuous implicit representation framework for \textbf{UHR} image segmentation. Specifically, we follow the basic manner in \textbf{LIIF} to align the input and refinement target continuously. The features are first projected into the desired resolution. Then an implicit function combines position information and aligned latent image features to predict the segmentation label for the queried pixel on images. To supervise the Transformer-based feature extractor, we generate the affinity label from ground truth to supervise the semantic affinity learned from the multi-head self-attention in the Transformer.

% Building on the preceding analysis, we propose a Transformer-based continuous implicit representation framework for \textbf{UHR} image segmentation. Specifically, The process begins by projecting features into the desired resolution. Subsequently, an implicit function integrates position information with the aligned latent image feature to predict the segmentation label for each queried pixel. To guide the Transformer-based feature extractor, we generate the affinity labels from ground truth to supervise the semantic affinity learned from the multi-head self-attention in the Transformer.

%The prior image segmentation decoder employed a single MLP network with pairs of linear layers to upscale image features into a segmentation output. However, this approach led to a segmentation mask that was overly general and remained fixed when handling different object classes. To address this limitation, we introduced a parameterized MLP network of our own and developed an innovative CNN-based hypernetwork to learn the MLP's parameters. Building upon the foundational structure of vanilla MLP and linear layers, the novel MLP network integrates both positional coordinate information and aligned latent image features to forecast the segmentation label for a queried pixel within the images. The hypernetwork utilizes convolutional layers to incorporate local patterns and spatial information from the entire input image. This enables us to effectively recognize and adaptively select parameters tailored to different segmentation object classes. As a result, this segmentation network exhibits greater adaptability compared to the previous MLP decoder, leading to a significant enhancement in segmentation precision.

% To overcome the limitations of prior image segmentation decoders that used a single MLP network with linear layer pairs for upscaling image features into a segmentation output, we have developed an innovative approach. We introduced a parameterized MLP network and designed a novel CNN-based hypernetwork to learn the MLP's parameters. Our advanced MLP network, built upon the fundamental structure of vanilla MLP and linear layers, integrates positional coordinate information and aligned latent image features. This integration is key to accurately forecasting the segmentation label for a queried pixel within images. 
% The hypernetwork, employing convolutional layers, captures local patterns and spatial information from the entire input image. This allows it to effectively recognize and adaptively select parameters that are specific to different segmentation object classes. Consequently, our segmentation network shows enhanced adaptability compared to the previous MLP decoder, resulting in a marked improvement in segmentation precision.

% Our main contribution is the following.
% \begin{itemize}
%     \item We propose a novel approach for \textbf{UHR} image segmentation using Adaptive Implicit Representation (AIR). The AIR method allows for flexible and precise mapping of pixel-level features, addressing the issue of traditional methods neglecting global semantic information.
%     \item We have developed a robust feature extractor (\textbf{Affinity Empowered Encoder}) that combines the advantages of transformer architecture and semantic affinity to model long-distance features effectively. This encoder enhances the accuracy and robustness of feature extraction by learning and utilizing semantic affinity.
%     \item We propose an \textbf{Adaptive Implicit Mapping Function} for flexible and precise mapping of pixel-level features. This function enables more detailed and individualized feature mapping, thereby improving the accuracy and effectiveness of segmentation.
%     %\item As far as we are aware, we are the first to introduce a CNN-based hypernetwork for learning the parameters of the segmentation decoder, resulting in improved adaptability and diversity of results across various input segmentations.
%     %\item We perform extensive experiments to demonstrate the effectiveness of \textbf{UHR} image segmentation, which outperforms other methods and contributes to the enhanced performance of cutting-edge panoptic segmentation models without requiring additional fine-tuning.
% \end{itemize}

==> Ziyu_Zhao_cvpr2024/sec/3_Experiments.tex <==


\section{Experiments}
%In this section, we we perform both quantitative and qualitative assessments of our results with relabeld PASCAL VOC 2012 \cite{Everingham2014ThePV} and BIG \cite{cheng2020cascadepsp} datasets respectively. We evaluate our model via Intersection over Union (IoU) and mean Boundary Accuracy (mBA) \cite{cheng2020cascadepsp}, which robustly computes the segmentation accuracy across different image sizes within a specified radius from the ground truth boundary. We evaluate our model without resorting to finetuning in various settings and demonstrate the enhancements achieved by our model.
%
\subsection{Setups}
%
{\bf Datasets.} To acquire object information and evaluate our models, we adhere to a dataset setup similar to that of CascadePSP \cite{cheng2020cascadepsp}. Our training dataset comprises a combination of several individual datasets, totaling 36,572 RGB images accompanied by their corresponding ground truth masks. These images encompass a wide spectrum of over 1,000 categories, drawing from MSRA-10K \cite{6871397}, DUT-OMRON \cite{6619251}, ECSSD \cite{7182346}, and FSS-1000 \cite{Wei2019FSS1000A1}. For testing, CascadePSP introduced a high-resolution image segmentation dataset, named BIG, ranging from 2K to 6K. Additionally, recognizing that the commonly used original PASCAL VOC 2012 dataset lacks pixel-perfect segmentations and designates regions near object boundaries as 'void', \cite{cheng2020cascadepsp} relabeled 500 objects to create a new dataset suitable for the task of \textbf{UHR} image segmentation.

{\bf Metrics.} We evaluate our model using Intersection over Union (IoU) and mean Boundary Accuracy (mBA) \cite{cheng2020cascadepsp}, which robustly computes the segmentation accuracy across different image sizes within a specified radius from the ground truth boundary. Our model is evaluated without resorting to finetuning in various settings, demonstrating the enhancements it achieves.


% {\bf Baselines.}














\subsection{Quantitative Results}

 Table \ref{quantitative} provides a comprehensive comparison of class-agnostic IoU and mBA among our \textbf{AIRM}, SegFix \cite{yuan2020segfix}, CascadePSP \cite{cheng2020cascadepsp} and CRM \cite{shen2022high}. All models are trained on low-resolution images and evaluated on their original high-resolution counterparts. Across both datasets, our method consistently outperforms other methods in terms of IoU and mBA. It's worth noting that SegFix's refinement performances are comparatively lower, as it is not specifically designed for the UHR image segmentation task. In the BIG dataset, our method exhibits an average improvement of around 1.7\% for IoU and 1.2\% for mBA based on four fundamental segmentation approaches. Similarly, in the relabeled PASCAL VOC 2012 dataset, our method achieves an average increase of approximately 1.1\% for IoU and 0.6\% for mBA compared to CRM and CascadePSP upon four approaches. These quantitative findings underscore the effectiveness of our model in capturing global semantic features and exploring pixel-wise affinity interrelationships in \textbf{UHR} image segmentation.

\begin{figure*}[t]
\centering
    {\includegraphics[width=1.0\linewidth]{images/qualitative.pdf}}
    \vspace{-15pt}
    \caption{Qualitative comparison of CascadePSP, CRM and \textbf{AIR} on the coarse masks from DeepLabV3+, RefineNet, PSPNet and FCN-8s. The images are from BIG dataset (2K$\sim$6K). The binary mask in the top-left part of the first column represents the ground truth.}
    \label{big}
    \vspace{-10pt}
\end{figure*}

\subsection{Qualitative Results}

In \figref{big}, we present a qualitative comparison of the performance of CascadePSP, CRM, and our \textbf{AIRM}. Remarkably, even without any prior exposure to high-resolution training images, our method consistently produces refined results of exceptional quality across various scales. When employing four distinct input coarse masks, it becomes evident that our approach excels at reconstructing missing parts in comparison to CascadePSP and CRM. For instance, as depicted in \figref{big}, our method accurately distinguishes the pilot and the passenger seated in the rear of the aeroplane (the second row) from the segmented object. Additionally, our method precisely delineates the shape of the right rear-view mirror (the third row), achieving a notably high level of precision when compared to the ground truth, which other methods fail to accomplish.

Furthermore,  \figref{Voc} underscores the substantial visual enhancements achieved by our refinement technique on the relabeled PASCAL VOC 2012 dataset, which consists of low-resolution images. A direct comparison highlights the generation of finer details in our outputs, particularly along the boundary region, such as the gap in the back of the chair and intricate feather textures. More results in supplementary material further demonstrate the efficacy of our refinement algorithm.



\begin{figure}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{images/voc.pdf}

   \caption{Qualitative output between CRM and our refinement algorithm on PASCAL VOC 2012 dataset(left to right). Coarse masks are from DeepLabV3+.}
   \label{Voc}
   \vspace{-5pt}
\end{figure}




\subsection{Ablation Study}


{\bf Affinity learning.}
\figref{affinity} illustrates that the attention map \figref{affinity} (b) can only represent the coarse-level semantic affinity relations, prompting us to investigate the reliable semantic affinities \figref{affinity} (c). 
In Table \ref{w/o}, we showcase the implementation of affinity learning across diverse backbones. For simplicity, We follow the method in \cite{ahn2018learning} to acquire the affinity prediction map in CNN-based backbone. In this approach, the semantic affinity between a pair of feature vectors is defined in terms of their L1 distance. Notably, leveraging affinity from attention within the Transformer encoder yields a performance boost, averaging 1.8\%/3.2\% higher than its counterpart in the CNN-based encoder. This outcome strongly validates both our initial motivation and the effectiveness of the AEE module.

 \begin{table}
 \renewcommand{\arraystretch}{0.93}
  \centering
  \setlength{\tabcolsep}{12pt}
  \begin{tabular}{ccc}

    \toprule
    Backbone & w Affinity  & w/o Affinity \\
    \midrule
    R50 &90.14/68.29& 89.99/67.96 \\ 
    \linespread{2}
    R101 &90.57/72.19& 90.03/72.99\\
    \linespread{2}
    WR38        &90.99/70.67& 90.84/69.11\\
    Mit-B1(Ours) &92.99/74.77& 91.25/72.96 \\
    \bottomrule
  \end{tabular}
  \vspace{-5pt}
  \caption{The effect of affinity learning based on various backbone via IoU/mBA(\%). R50, R101 and WR38 denote the method used in ResNet50, ResNet101 \cite{he2016deep} and WideResNet38 \cite{wu2019wider}. The results are evaluated on the BIG dataset. Coarse masks are from DeepLabV3+.}
  \label{w/o}
  \vspace{-15pt}
\end{table}


\begin{figure}[bt]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{images/affinity.pdf}

   \caption{Visualization of attention map and affinity. }
   \label{affinity}
   \vspace{-5pt}
\end{figure}

\begin{figure}[bt]

% \vspace{-21pt}
\centering
\includegraphics[width=1\linewidth]{images/adaptive.pdf}
\caption{Visualization of the adaptive parameters.}
\vspace{0pt}
\label{adaptive}
\end{figure}




{\bf Adaptive implicit representation mapping function.}
We employ the TSNE \cite{van2008visualizing} to reduce the dimension of the predicted adaptive parameters and illustrate that in \figref{adaptive}. We observe that for input images with a similar semantic appearance, the corresponding mapping parameters are closely related. This demonstrates that the predicted adaptive parameters possess the capability to capture global semantic information.

\begin{table}[bt]
\renewcommand{\arraystretch}{0.93}
  \centering
  \setlength{\tabcolsep}{12pt}
  \begin{tabular}{cccc}
    \toprule

    AEE & AIRMF& IoU & mBA \\
    \midrule
    \ding{56}& \ding{56}& 88.75  & 68.34\\
    \ding{52}& \ding{56}  & 90.99 & 70.77\\
    \ding{56}& \ding{52} &  91.08 &  71.09      \\
    \ding{52}& \ding{52} &   92.99 &  74.77   \\
    \bottomrule
  \end{tabular}
  \vspace{-5pt}
  \caption{The ablation study about AEE and AIRMF. Note that we utilize ResNet50 \cite{he2016deep} as the substitute encoder and SIRMF (a standard 5-layer MLP) as the alternative implicit function in the ablation study. The results are evaluated on the BIG dataset. Coarse masks are from DeepLabV3+.}
  \label{AIR}
\vspace{-15pt}
\end{table}
Table \ref{AIR} showcases the effect of the presence of AIRMF. For a fair comparison, we adopt ResNet50 \cite{he2016deep} as an alternative image encoder for extracting image features when AEE is not employed. Additionally, we utilize a naive 5-layer MLP network as the substitute implicit function for AIRMF to decode the extracted latent code, following the setup outlined in \cite{chen2021learning}. As shown in Table \ref{AIR}, we have the following observations: \ding{182} Without our proposed empowered encoder and adaptive implicit function, the segmentation results decrease by 2.24\%/2.43\% and 2.33\%/2.75\%, respectively, compared with a CNN-based encoder and conventional implicit function (see the first-third rows). This highlights our empowered encoder can efficiently capture strong and dependable global semantic information than the CNN-based encoder. Furthermore, our adaptive implicit function effectively utilizes these global features to compute the adaptive parameters, cooperatively enhancing segmentation performance. \ding{183} Particularly noteworthy is the synergistic performance achieved by the cohesive implementation of both modules in our proposed method, achieving the highest performance at 92.99\%/74.77\% (see the fourth row). This underscores the essential roles of AEE and AIRMF within AIRM, showcasing their synergistic effects.  


% The results reveal superior performance for our proposed AEE and AIRMF modules, surpassing the original module by 2.24\%/2.43\% and 2.33\%/2.75\%, respectively.  Particularly noteworthy is the synergistic performance achieved by the cohesive implementation of both modules in our proposed method, achieving the highest performance at 92.99\%/74.77\%. This underscores the essential roles of AEE and AIRMF within AIRM, showcasing their synergistic effects.

% Essentially, the affinity loss aims to compel the encoder to acquire strong, dependable semantic affinity relationships through the multi-head self-attention map. Moreover, as the affinity prediction $\mathbf{Aff}_{pre}$ is derived as a linear combination of attention map, this loss function also contributes to the improvement of self-attention learning and facilitates the identification of integral object regions.







{\bf Search mask radius in affinity loss.}
In Table \ref{radius}, we also study the segmentation performance on different search mask radius $R$ when generating affinity label for computing affinity loss. Through comparison, we observe that a small value of $R$ may not yield sufficient affinity pairs, whereas a large 
$R$ might compromise the reliability of distant affinity pairs. Thus, we choose $R$ = 14 as our priority.

\begin{table}[]
 % \renewcommand{\arraystretch}{0.93}
	\centering
	\renewcommand\arraystretch{1.5}
	\setlength{\tabcolsep}{1.5mm}{
		\begin{tabular}{c|c|c|c|c|c}
		    \hline
		    $R$ & 6 & 10 & \textbf{14} & 18 & 20\\
		    \hline
		    IoU& 91.28&91.38& \textbf{91.47}&90.99&90.85\\
		    \hline
    	\end{tabular}}
            \vspace{-5pt}
     	\caption{Ablation study on radius $R$ of the affinity loss. The results are evaluated on the BIG dataset. Coarse masks are from DeepLabV3+.}
      \label{radius}
        \vspace{-10pt}
\end{table}


\section{Conclusion}
% We propose \textit{Adaptive Implicit Representation Mapping} (AIRM), a general framework for high-resolution image segmentation. AIRM leverages the Transformer architecture with semantic-level affinity to effectively extract latent embeddings. Additionally, our approach incorporates an adaptive implicit function, dynamically blending global semantic information with pixel-wise features to convert features into segmentation values. Extensive experiments validate the superior performance of our method, surpassing competitors by a significant margin.

Our study dives deep into how receptive fields influence implicit representation mapping and explores the shortcomings of current shared mapping functions through extensive experiments. Building on our findings, we introduce an innovative approach titled "Leveraging Adaptive Implicit Representation Mapping for Ultra-High-Resolution Image Segmentation." This paradigmatic framework comprises two integral components: the Affinity Empowered Encoder (AEE) and the Adaptive Implicit Representation Mapping Function (AIRMF). Together, this methodological approach facilitates the extraction of pixel-wise features with a much larger receptive field, translating it into a segmentation result enriched with global semantic information. Our meticulous experimentation substantiates the remarkable efficacy that our approach outperforms competitors by a significant margin. 
%
Fundamentally, we are shedding light on the limitations of existing methods and offering a promising avenue for ultra-high-resolution image segmentation with improved accuracy and performance.

==> Ziyu_Zhao_cvpr2024/sec/Discussion.tex <==
%-----------------------------------------------------
\begin{figure}[b]
\vspace{-15pt}
\centering
\includegraphics[width=1.0\linewidth]{images/discussion.pdf}
\captionsetup{font={small}}
\caption{
\vspace{0pt}
(a) The impact of receptive fields on IRM. The blue points and red points denote the SIRMF and AIRMF respectively (b) Analyze the limitation of the existing SIRMF. The blue bar denotes one SIRMF on three categories, the yellow bar denotes the three SIRMF on each category respectively, and the red bar denotes the AIRFM. 
}
\vspace{0pt}
\label{fig:dis}
\end{figure}
%-----------------------------------------------------
%
\section{Discussion and Motivation}
\label{dis_moti}
%
% Since we argued that the size of receptive fields can significantly impact the performance of the IRM and the SIRMF lacks the generalization capability to handle diverse inputs, 

In this section, we conduct several comprehensive experiments to explore the impact of receptive fields on IRM 
(see \secref{receptive_fields}) and analyze the limitation of the existing SIRMF (see \secref{limitation_ip}). 
We observe that (1) larger receptive fields significantly enhance the performance of IRM, and (2) the existing SIRMF lacks the generalization capability to handle diverse inputs and tends to overlook global semantic information. Building on these observations, we introduce a novel approach named \textit{Leveraging Adaptive Implicit Representation Mapping for Ultra-High-Resolution Image Segmentation}.
%These experiments are conducted based on a standard UHR image segmentation pipeline as illustrated in Figure \ref{fig:fig1}a, where it contains a CNN-based Encoder to extract image features, followed by a SIRMF to predict the segmentation results.
%
\subsection{The Impact of Receptive Fields on IRM}
\label{receptive_fields}
%
{\bf Image encoder.} To investigate the impact of receptive fields on IRM, we construct a straightforward image encoder, \ie $\phi$, comprising only several convolutional layers, followed by ReLU and batch normalization operations. We then utilize the encoder $\phi$ to extract features $\mathbf{F} \in \mathbb{R}^{h \times w \times D}$ from the input image $\mathbf{I}$ and coarse segmentation mask $\mathbf{M}$,
%
%--------------------
\begin{align}
   \mathbf{F} = \phi(\mathbf{I}, \mathbf{M}).
\end{align}
%--------------------
%

{\bf SIRMF.} Following \cite{chen2021learning}, the SIRMF is implemented by an MLP network, denotes as $\textit{f}_\theta$, and the refined segmentation result $\Tilde{\mathbf{M}}_{q}$ at location ${q}$, can be represented as
%
%--------------------
\begin{align}
    \label{liff}
   \Tilde{\mathbf{M}}_{q} = \sum_{p \in \mathcal{N}_q} \frac{S_p}{\sum{S_p}} \cdot \textit{f}_\theta(z_p, p - q),
\end{align}
%--------------------
%
where $\textit{f}$ is the mapping function, $\theta$ is the trainable parameter of $\textit{f}$,  $\mathcal{N}_q$ are neighbor locations around $q$, and $z_p$ is the pixel-wise feature vector related to location $p$. The aggregation weights, \ie area value $\mathbf{S}_p$ are calculated based on the relative coordinate offset between $q$ and $p$.
% and $\mathbf{S}$ is the sum areas of all $p$.
%

We train the image encoder $\phi$ with various kernel sizes and the SIRMF $\textit{f}_{\theta}$ on the high-resolution image segmentation dataset. Subsequently, we evaluate the performance based on the Intersection over Union (IoU) and illustrate the results in \figref{fig:dis} (a) (see the blue line). We can observe a substantial performance improvement in the segmentation results when enlarging the kernel size. This highlights that larger receptive fields significantly enhance the performance of IRM in the context of image segmentation tasks.
%
%

\begin{figure*}[t]
	\begin{center}
	    \includegraphics[width=1\linewidth]{images/pipeline.pdf} 
            \captionsetup{font={small}}
            \vspace{-20pt}
		\caption{The proposed architecture of \textbf{AIRM}. We employ an affinity-empowered encoder (AEE) to extract the image features. Then we utilize the adaptive implicit representation mapping function (AIRMF) to adaptively translate pixel-wise features without neglecting global semantic information.
  } 
		\label{main}
		\vspace{-20pt}
            \label{pipeline}
	\end{center}

\end{figure*}

\subsection{Limitation of The existing SIRMF}
\label{limitation_ip}
%
To further analyze the limitations of the current SIRMF, we randomly select three categories of images from the segmentation dataset. Subsequently, we conduct the following experiments: 

{\bf Exp.1} We utilize the pre-trained image encoder $\phi$ from \secref{receptive_fields} to extract image features. We train a SIRMF on the entire selected image set and then evaluate the performance of the SIRMF on each category separately (see \figref{fig:dis} (b) blue bar). 

{\bf Exp.2} We use the same encoder as in Exp.1 to extract image features. But we train three SIRMF, each dedicated to one of the selected categories, and then evaluate the performance of each SIRMF on its corresponding category (see \figref{fig:dis} (b) yellow bar). 

From \figref{fig:dis} (b) we can observe that training three SIRMF separately for each category yields better performance compared to training one SIRMF across all three categories. This observation indicates that the existing SIRMF lacks the generalization capability to effectively handle specific categories and tends to overlook global semantic information.






==> Ziyu_Zhao_cvpr2024/sec/Methodology.tex <==


\section{Methodology}
% This section first describes the general framework of our \textbf{UHR} image segmentation network in Sec(), then explains the transformer-based affinity learning and hypernetwork leveraged in adaptive implicit function, in Sec () and Sec () respectively.
%
Building upon the observations in \secref{dis_moti}, in this section, we introduce a novel approach that leverages adaptive implicit representation mapping for ultra-high-resolution image segmentation to effectively address the previous limitations, as shown in \figref{pipeline}. Specifically, the proposed method \textbf{AIRM} comprises two components: the Affinity Empowered Encoder (\textbf{AEE}) (see \secref{encoder}) and the Adaptive Implicit Representation Mapping Function (\textbf{AIRMF}) (see \secref{mapping}). The AEE is responsible for effectively modeling long-distance features by taking advantage of the transformer architecture and semantic affinity. The AIRMF is responsible for adaptively translating pixel-wise features without neglecting the global semantic information, allowing for flexible and precise feature translation.

% \subsection{Method Overview}
% \figref{pipeline} illustrates the overall structure of our proposed method.  Given an RGB image, we start by concatenating it with the initial coarse mask, creating 4-channel input denoted as $I_M \in \mathbb{R}^{4 \times H \times W}$. This input is then encoded into a latent embedding $F \in \mathbb{R}^{C \times h \times w}$ through our novel Affinity Empowered Encoder (AEE) $E_\theta$. 
% Following this, $F$ is processed by our Adaptive Implicit Representation Mapping Function (AIRMF) decoder $D_\phi$ to generate the final results at the original size.

%Then, $F$ is processed by our innovative Adaptive Implicit Mapping Function (AIMF) decoder $D_\phi$ to produce the final results at the original size. 


\subsection{Affinity Empowered Encoder}
\label{encoder}
%
% Figure \ref{pipeline} demonstrates an overview of our network architecture, the general architecture can be described as an encoder part (in blue) and a decoder part (in orange). For a given RGB image, we firstly concatenate it with the initial coarse mask as 4-channel input $I_M \in \mathbb{R}^{4 \times H \times W}$. A Transformer based encoder will encode the concatenated input to 2D grid feature maps at different levels. The affinity map will be computed upon the multi-head self-attention maps in each block. For the decoder part, after the encoder builds a top-down pathway
% with bilinear up-sampling, our method proposed a hypernetwork to adaptively map these feature embeddings into segmentation signals at every coordinate parallelly.

%  forming a point-independent prediction manner.


% \subsection{Feature Alignment Function}







% \subsection{Affinity Transformer}

% Let us first revisit the affinity learning proposed in \cite{ru2022learning}, which deals with a weakly-supervised semantic segmentation task. In this scenario, where ground truth labels are absent, the method draws inspiration from the consistency between the multi-head self-attention (MHSA) in the Transformer model and the semantic-level affinity.

%Considering the limitations of the CNN network in capturing long-range dependencies and the limited receptive field mentioned above, we have taken the initiative to incorporate a Transformer-based encoder into this task. Nevertheless, no explicit constraints are applied to the self-attention matrices during the training phase. We take inspiration from \cite{ru2022learning} to investigate the alignment between the multi-head self-attention (MHSA) in the Transformer model and the semantic-level affinity. In light of this,  we propose to learn the affinity from MHSA to intentionally impose constraints on our encoder during the training.  

As discussed in \secref{dis_moti}, larger receptive fields significantly enhance the performance of IRM. Therefore, instead of employing a CNN-based image encoder like CRM \cite{shen2022high} and LIIF \cite{chen2021learning}, we propose an affinity-empowered image encoder that takes advantage of the transformer architecture and semantic affinity.
%
Specifically, given the RGB image $\mathbf{I} \in \mathbb{R}^{H \times W \times 3}$ and the corresponding coarse segmentation mask $\mathbf{M} \in \mathbb{R}^{H \times W \times 1}$, we employ the transformer-based encoder $\omega$ to extract features $\mathbf{F}$, which can be represented as follows:
%
\begin{equation}
    \mathbf{F}, \mathbf{ATT} = \omega(\mathbf{I}, \mathbf{M}),
\end{equation}
%
where $\mathbf{ATT} \in \mathbb{R}^{hw \times hw \times c}$ denotes the attention map produced by $\omega$ and $hw$ represents the flattened spatial dimensions and $c$ is the number of channels. Note that the coarse segmentation mask is obtained by applying an existing segmentation method such as \cite{long2015fully, chen2018encoder, lin2017refinenet}.
%

% Next, recognizing the consistency between the multi-head self-attention map in the transformer and the semantic-level affinity, we leverage the affinity to augment our encoder with ample semantic information.

To further empower the capability of the transformer-based encoder, we propose learning the affinity from the attention map $\mathbf{ATT}$ to intentionally impose constraints on the encoder $\omega$ during training. 
%
% The affinity matrix is derived from the attention map $\mathbf{ATT}$.
%
% should possess symmetry, given the points with identical semantic information are expected to share equal values. Therefore, 
%
Specifically, we obtain the predicted affinity $\mathbf{Aff}_{pre}\in \mathbb{R}^{hw \times hw}$ by feeding the sum of $\mathbf{ATT}$ and its transpose into an MLP network, \ie, $\varphi$, which can be represented as: 
\begin{equation}
    \mathbf{Aff}_{pre} = \varphi(\mathbf{ATT} + \mathbf{ATT}^\top).
\end{equation}
We expect $\mathbf{Aff}_{pre}$ to be close to the ground truth affinity $\mathbf{Aff}_{gt} \in \mathbb{R}^{hw \times hw}$ obtained from the ground truth segmentation mask $\hat{\mathbf{M}}$. Specifically, we resize $\hat{\mathbf{M}}$ to $hw \times hw$ to align with the shape of $\mathbf{Aff}_{gt}$ and the affinity between two coordinates $(x_i, y_i)$ and $(x_j, y_j)$ is assigned as 1 if their classes are identical, and 0 otherwise.




% Considering the limitations of CNNs in capturing long-range dependencies and their limited receptive field, we have incorporated a Transformer-based encoder into this task. However, the self-attention maps in the transformer lack semantic affinity information. Drawing inspiration from \cite{ru2022learning}, we explore the alignment between the multi-head self-attention (MHSA) in the Transformer model and the semantic-level affinity. Consequently, we propose learning the affinity from MHSA to intentionally impose constraints on our encoder during training.


% Particularly, the semantic affinity is derived by directly utilizing a linear MLP layer to the multi-head attention $S \in \mathbb{R}^{hw \times hw \times n}$, where $hw$ represents the flattened spatial dimensions and $n$ is the number of attention heads. Specifically, this process involves adding $S$ and its transpose to predict the semantic affinity matrix $W \in \mathbb{R}^{hw \times hw}$ as below:

% \begin{equation}
%     W = {\rm \textbf{MLP}}(S + S^{T})
% \end{equation}
% , where $S^{T}$ denotes the transpose of self-attention matrix in tensor $S$.
 

% Assuming MHSA in a Transformer block is represented as $S \in \mathbb{R}^{hw \times hw \times n}$, where $hw$ denotes the flattened spatial size and n is the number of attention heads. We generate the semantic affinity directly by applying a linear combination to the multi-head attention. Specifically, the self-attention mechanism resembles a directed graphical model [43], and the affinity matrix should exhibit symmetry since nodes that share the same semantics are expected to be equal. To achieve this transformation, we simply add $S$ and its transpose. The predicted semantic affinity matrix $W \in \mathbb{R}^{hw \times hw}$ is thus denoted as
% \begin{equation}
%     W = {\rm \textbf{MLP}}(S + S^{T})
% \end{equation}
%





\subsection{Adaptive Implicit Representation Mapping Function (AIRMF)}
\label{mapping}

% Due to the aforementioned drawbacks of vanilla MLP, we propose a hypernetwork $\mathcal{H}_{\Phi}$ to produce adaptive weights to map features $\textbf{f}_{\rm IR}$ into detailed segmentations. 

% Specifically, we first define a shared

% Based on the observation on \secref{limitation_ip}, 

% To attain high-resolution image segmentation, a critical challenge involves the integration of information from multi-level feature maps originating at various resolutions. Traditionally, the use of up-sampling modules is common to standardize these maps to a consistent resolution. However, our novel approach introduces the concept of continuous feature maps, which are essentially fields of features that can be decoded at any desired coordinates. This innovation facilitates seamless alignment within a continuous field, obviating the need for up-sampling.

% To define a continuous feature map $F$, we adopt the basic architecture of implicit feature function in LIIF []. In this framework, we treat the feature vectors in the discrete feature map as latent codes, evenly distributed in a 2D space, each associated with a unique 2D coordinate. We then integrate the feature map with the positional information of these coordinates and the feature-to-target ratio denoted as $r$. Therefore, for a given input $I_M$, with latent codes $z \in \mathbb{R}^{h \times w \times D}$ and query coordinate $x_q$, the target feature value of $F$ at $x_q$ is defined by:
% \begin{equation}
%     F_{\rm x_q} = \rm {Concate} [z^{*} , v^{*}, x_q - v^{*}, r],
% \end{equation}
% where $z^{*} \in \mathbb{R}^{H \times W \times D}$ is the nearest projected latent code from $x_q$ and $v^{*}$ is the coordinate of latent code $z^{*}$ .The feature $F_{\rm x_q}$ with the target size is of dimensions $\mathbb{R}^{H \times W \times (D+6)}$ and is subsequently input into the decoder.

In \secref{limitation_ip}, we identified the limitation in the existing SIRMF \eqref{liff} — it lacks the capacity to effectively generalize across diverse inputs (see \figref{fig:dis} (b)). To tackle this issue, we introduce SIRMF which can be represented as
%
%--------------------
\begin{align}
    \label{our_liff}
   \Tilde{\mathbf{M}}_{q} = \sum_{p \in \mathcal{N}_q} \frac{S_p}{\sum{S_p}} \cdot \textit{f}_{\psi(\mathbf{F})}(z_p, p - q),
\end{align}
%--------------------
%
where $\psi(\cdot)$ denotes a hypernetwork that is used to predict the adaptive mapping parameters.
%
Instead of directly optimizing the shared parameter $\theta$ in \eqref{liff}, we employ $\psi$ to predict it adaptively by inputting the feature $\mathbf{F}$. Intuitively, the predicted mapping parameter should capture global semantic information from the input feature $\mathbf{F}$. 
%
Consequently, AIRMF can leverage both local information from pixel-wise features and global information from the entire image feature. This design allows AIRMF to yield precise segmentation results (see the red points in \figref{fig:dis} (a) and the red bar in \figref{fig:dis} (b)).
%

Assume we aim to generate the weight ${\textit{\textbf{W}}^\textit{l}} \in \mathbb{R}^{n_{\rm in} \times n_{\rm out}}$ and bias ${\textit{\textbf{b}}^\textit{l}} \in \mathbb{R}^{n_{\rm out}}$ of the \textit{l}-th linear layer of $f(\cdot)$. To optimize computational efficiency, we do not directly predict the parameter. Instead, we adopt a strategy similar to \cite{skorokhodov2021adversarial}, predicting two intermediary rectangular  matrices ${\textit{\textbf{A}}^\textit{l}} \in \mathbb{R}^{n_{\rm out}^l \times r}$  and ${\textit{\textbf{B}}^\textit{l}} \in \mathbb{R}^{{r \times n_{\rm in}^l}}$  through $\psi(\cdot)$, where r = 20 for all the layers of $\textit{f}{(\cdot)}$. The linear modulating projection weight ${\textit{\textbf{W}}}^l$ is then modulated by multiplying these matrices as follow, 
\begin{equation}
    {\textit{\textbf{W}}}^l = {\textit{\textbf{A}}^\textit{l}} \times {\textit{\textbf{B}}^\textit{l}}.
\end{equation}
Bias parameter ${\textit{\textbf{b}}^\textit{l}}$ is directly produced due to its small volume. We streamline the AIRMF in \figref{pipeline}. 


% After the encoder stage, the size of the encoded feature is smaller than the refinement target. For our UHR image segmentation task, it's necessary to up-sample the intermediate feature or refine results for subsequent decoding. We adopt the Continuous Alignment Module approach proposed in [], which dynamically maps the low-resolution feature embedding to the target size. Typically, we sample extracted feature vectors on a 2D grid matching the target size and integrate them with the 2D target grid's coordinates and the relative target coordinate offset. 

% Therefore, for a given input $I_M$, with latent codes $F \in \mathbb{R}^{C \times h \times w}$ and query coordinate $x_q$, the target feature value of $F_{target}$ at $x_q$ is defined by:
% \begin{equation}
%     F_{\rm x_q} = \rm {Concate} [z^{*} , v^{*}, x_q - v^{*}, r],
% \end{equation}
% where $F^{*} \in \mathbb{R}^{D \times H \times W}$ is the nearest projected latent code from $x_q$ and $v^{*}$ is the coordinate of latent code $z^{*}$ .

\subsection{Implementation Details}

{\bf Network architectures.} We employ the Mix Transformer (MiT) introduced in Segformer \cite{xie2021segformer}) as the backbone of image encoder $\omega$. MiT is a more suitable backbone for image segmentation tasks compared to the vanilla ViT \cite{dosovitskiy2020image}. In brief, MiT incorporates overlapped patch embedding to maintain local consistency, spatial-reductive self-attention to accelerate computation, and employs FFN with convolutions to safely replace position embedding. The network of $\phi$ to predict the semantic affinity is implemented by an MLP layer. 
The deep network $\psi$ employed to generate the flattened parameters of the mapping function $\textit{f}(\cdot)$ is constructed by several \textit{Conv+ReLU+BatchNorm} layers, followed by a linear layer.

{\bf Loss.}
During training, we use the combined loss functions to optimize overall performance. To improve AIRMF, we utilize the cross-entropy loss $\mathcal{L}_{ce}$, L1 loss $\mathcal{L}_{1}$, L2 loss $\mathcal{L}_{2}$ and gradient loss $\mathcal{L}_{grad}$
\begin{equation}
    \mathcal{L}_{AIRMF} = \lambda_1\mathcal{L}_{1} + \lambda_2\mathcal{L}_{2} + \lambda_3\mathcal{L}_{ce} +\lambda_4\mathcal{L}_{grad},
\end{equation}
where $\lambda_1=0.2$, $\lambda_2=0.2$, $\lambda_3=0.3$ and $\lambda_4=0.4$ balance the contributions in $\mathcal{L}_{AIRMF}$.

%For computing the affinity loss $\mathcal{L}_{aff}$, we limit our focus to adjacent coordinates during training, leveraging their sufficient context and minimizing computational costs. Consequently, we employ a search mask on $\hat{\mathbf{M}}$ with a predefined radius of $R$ as a threshold, efficiently constraining the distance between selected pairs of coordinates. As a result, we exclusively consider pixel pairs situated within the same local search mask, disregarding the affinity between pixel pairs that are far apart. The affinity loss term is formulated as:

To calculate the affinity loss $\mathcal{L}_{aff}$, we concentrate on adjacent coordinates during training to leverage their sufficient context while minimizing computational costs. We use a search mask on $\hat{\mathbf{M}}$ with a predefined radius $R$ as a threshold, efficiently limiting the distance between selected coordinate pairs. This approach ensures that only pixel pairs within the same local search mask are considered, excluding the affinity between distant pixel pairs. The affinity loss term is formulated as follows:

\begin{equation}
\begin{aligned}
    \mathcal{L}_{aff} &= - \frac{1}{\lvert \mathcal{S}^{-} \rvert} \sum_{(i,j) \in \mathcal{S}^{-}} \log{(1-\mathbf{Aff}_{pre}^{i,j})} \\ 
    &- \frac{1}{\lvert \mathcal{S}^{+} \rvert} \sum_{(i,j) \in \mathcal{S}^{+}} \log {(\mathbf{Aff}_{pre}^{i,j})},
\end{aligned}
\end{equation}
where $\mathcal{S}^{+}$ and $\mathcal{S}^{-}$ refer to two subsets of positive and negative affinity pixel pairs: 
\begin{equation}
    \mathcal{S}^{+} = \{{(i,j) \mid (i,j) \in \mathcal{P}, \mathbf{Aff}_{pre}^{i,j} = 1}\},
\end{equation}
\begin{equation}
    \mathcal{S}^{-} = \{{(i,j) \mid (i,j) \in \mathcal{P}, \mathbf{Aff}_{pre}^{i,j} = 0}\}.
\end{equation}
Our final loss can be written as:
\begin{equation}
\begin{aligned}
    \mathcal{L}= \frac{1}{2}\mathcal{L}_{AIRMF} + \frac{1}{2}\mathcal{L}_{aff}.
\end{aligned}
\end{equation}



\begin{table*}[bt]
\renewcommand{\arraystretch}{1}
	\centering
        \setlength{\tabcolsep}{12pt}
	%\renewcommand\arraystretch{1.5}
	% \setlength{\tabcolsep}{1.5mm}
        \begin{tabular}{cccccc}
            \toprule
            IoU/mBA(\%)&Coarse Mask&  SegFix \cite{yuan2020segfix}    & CascadePSP \cite{cheng2020cascadepsp} & CRM \cite{shen2022high}& AIRM(Ours)\\
            \midrule
            % \midrule
            \multicolumn{6}{c}{\centering \textbf{BIG}}\\
            \midrule
            FCN-8s \cite{long2015fully}    &72.39/53.63 & 72.69/55.21  & 77.87/67.04& 79.62/69.47& \textbf{80.59}/\textbf{69.98}\\
            % \midrule
            RefineNet \cite{chen2018encoder} &90.20/62.03 & 90.73/65.95  & 92.79/74.77& 92.89/\textbf{75.50}& \textbf{93.59}/75.26\\
            % \midrule
            DeepLabV3+ \cite{lin2017refinenet}&89.42/60.25 & 89.95/64.34  & 92.23/74.59& 91.84/\textbf{74.96}& \textbf{92.99}/74.77\\
            % \midrule
            PSPNet \cite{zhao2017pyramid}   &90.49/59.63 & 91.01/63.25  & 93.93/75.32& 94.18/76.09& \textbf{94.95}/\textbf{76.88}\\
            % \midrule
            \midrule
            \multicolumn{6}{c}{\centering \textbf{PASCAL VOC 2012}}\\
            \midrule
            FCN-8s \cite{long2015fully}    &68.85/54.05 & 70.02/57.63  & 72.70/65.36& 73.34/67.17& \textbf{74.59}/\textbf{67.26}\\
            % \midrule
            RefineNet \cite{chen2018encoder}&90.20/62.03 & 86.71/66.15  & 87.48/71.34& 87.18/71.54& \textbf{88.03}/\textbf{71.89}\\
            % \midrule
            DeepLabV3+ \cite{lin2017refinenet}&87.13/61.18 & 88.03/66.35  & 89.01/72.10& 88.33/\textbf{72.25}& \textbf{90.01}/72.01\\
            % \midrule
            PSPNet \cite{zhao2017pyramid}    &90.92/60.51 & 91.98/66.03  & 92.86/72.24& 92.52/72.48& \textbf{93.56}/\textbf{73.39}\\
            \bottomrule
        \end{tabular}
        % \setlength{\abovecaptionskip}{.28cm}
        % \vspace{3pt}
        \captionsetup{font={footnotesize}}
        \vspace{0pt}
        \caption{Comparison of IoU and mBA results on BIG and PASCAL VOC 2012 datasets with varied mask refinement methods, utilizing coarse masks generated by FCN, RefineNet,  DeepLabV3+ and PSPNet. Optimal performances are indicated in bold.}
        \label{quantitative}
          \vspace{-0pt}
\end{table*}

{\bf Training details.} During training, we utilize the Adam optimizer \cite{kingma2017adam} with an initial learning rate $2.25 \times 10^{-5}$ to train our network. The learning rate is decayed to one-tenth at iterations 22,500 and 37,500 in a total of 45,000 iterations. We randomly crop input with a resolution of 224x224 from the original images. During the training, the coarse masks are generated by introducing random perturbations to the ground truth masks with a random IoU threshold ranging from 0.8 to 1.0. The radius $R$ of the local window size when computing the affinity loss is set to 14.

We follow the multi-resolution inference strategy proposed in \cite{shen2022high}, which can be seen as progressively coarse-to-fine operations. Specifically, the inference begins at a very low resolution around the training image resolution and gradually increases the input’s resolution along the continuous ratio axis $Rs \in (0.125,0.25,0.5,1)$. At each refinement stage, the refined mask is concatenated as a coarse mask for the next refinement step.





% \begin{figure*}[t]
% \centering
%     {\includegraphics[width=1.0\linewidth]{images/qualitative.pdf}}
%     \vspace{-15pt}
%     \caption{Qualitative comparison of CascadePSP, CRM and \textbf{AIR} on the coarse masks from DeepLabV3+, RefineNet, PSPNet and FCN-8s. The images are from BIG dataset (2K$\sim$6K). The binary mask in the top-left part of the first column represents the ground truth.}
%     \label{big}
%     \vspace{-10pt}
% \end{figure*}

==> Ziyu_Zhao_cvpr2024/sec/Related_Work.tex <==
\section{Related Work}
% \subsection{Semantic Segmentation}
% The progress in semantic segmentation, which involves assigning distinct categories or classes to individual pixels within an image, has been significantly propelled by the achievements of deep neural networks \cite{krizhevsky2012imagenet,simonyan2014very,lin2017feature}. FCNs \cite{long2015fully} extend the capabilities of CNNs by introducing upsampling layers, enabling pixel-level predictions, and enabling end-to-end segmentation. 
% However, the preceding approaches often produce output segmentation images with reduced resolution due to the numerous convolutional and pooling layers they employ. Further, they struggle to capture long-range dependencies of the feature maps. Previous \textbf{UHR} image segmentation methods \cite{cheng2020cascadepsp, xu2021hrcnet,
% hoyer2022hrda,
% wang2022semantic, shen2022high} commonly adopted CNN-based networks as their primary feature extractors. However, these approaches have posed limitations in capturing a broader receptive field, subsequently impacting the accuracy of segmentation results, especially in scenarios where fine details and aspect sensitivity are critical.
% Therefore, we propose leveraging attention mechanisms within Transformer architectures to effectively address these limitations and challenges.

\subsection{Refining Semantic Segmentation}

The progress in semantic segmentation, which aims to assign distinct categories or classes to individual pixels within an image, has been significantly propelled by the achievements of deep neural networks \cite{long2015fully,krizhevsky2012imagenet,simonyan2014very,lin2017feature, chen2017deeplab,chen2016attention, farabet2012learning, he2004multiscale,mostajabi2015feedforward,shotton2009textonboost,zhang2018context}. 
%FCNs \cite{long2015fully} extend the capabilities of CNNs by introducing upsampling layers, enabling pixel-level predictions, and enabling end-to-end segmentation. 
However, these methods are primarily focused on tackling the issue of low-resolution image segmentation but fall short of producing high-quality segmentation results. 
Thus,
%The philosophy behind refining segmentation 
the task of refining segmentation is introduced to improve the quality of segmentation outcomes for high-resolution (1K$\sim$2K) (\textbf{HR}) or even ultra high-resolution  (4K$\sim$6K) (\textbf{UHR}) images. Unlike low-resolution images, \textbf{HR} and \textbf{UHR} require a deeper understanding of semantic details. 
Conventional techniques rely on graphical models like CRF \cite{chen2014semantic,chen2017deeplab,
lin2016efficient, krahenbuhl2011efficient, liu2015semantic} or region growing \cite{dias2019semantic} techniques to achieve HR segmentation. But they mainly focus on low-level color boundaries \cite{zheng2015conditional}, limiting their segmentation performance. %Propagation-based techniques \cite{liu2017learning} struggle to effectively handle \textbf{UHR} data due to their inherent limitations in terms of computational expenses and memory constraints. 
In contrast, Multi-scale Cascade Networks \cite{chen2019collaborative, cheng2020cascadepsp, he2019bi, qi2018sequential, sun2013deep, zhao2018icnet} employ a recursive approach to progressively integrate multi-scale information. Nevertheless, such a recursive approach inadvertently introduces more computational burdens. Therefore, a Continuous Refinement Network \cite{shen2022high} is proposed to improve the efficiency by continually aligning the feature map with the refinement target. However, it tends to overlook the significance of the limited receptive field of the Convolution Operation in the CNN backbone and also lacks the generalization capability to effectively handle specific categories. To address these concerns, we employ a Transformer-based adaptive implicit representation function to mitigate these limitations and improve segmentation accuracy.

%-------------------------------------------------------------------------
\subsection{Transformer in Segmentation}

% When Vision Transformers (ViT) \cite{dosovitskiy2020image} were introduced, transformer-based deep networks demonstrated remarkable success, surpassing convolutional-based networks in various computer vision fields such as image restoration and detection.
%
Vision Transformers (ViT) \cite{dosovitskiy2020image}, as demonstrated by their remarkable success, is adapted for various computer vision tasks such as semantic segmentation \cite{liu2021swin, zheng2021rethinking} and object segmentation \cite{zhu2020deformable, dai2021dynamic}. 
%
However, applying plain Vision Transformer (ViT) models directly to segmentation tasks is challenging due to their absence of segmentation-specific heads. To solve this problem, SETR \cite{zheng2021rethinking} reframes semantic segmentation as a sequence-to-sequence prediction task. \cite{liu2021swin} proposes a versatile hierarchical Vision Transformer backbone, known as Swin Transformer (Hierarchical Vision Transformer using Shifted Windows), using shifted windows to efficiently capture long-range dependencies while maintaining scalability. Segmenter \cite{strudel2021segmenter} employs pre-trained image classification models fine-tuned on moderate-sized segmentation datasets for semantic segmentation tasks. 
%SegFormer \cite{xie2021segformer} consists of a hierarchical Transformer encoder with a lightweight multilayer perceptron (MLP) decoder. 
Instead of ViT, \cite{ru2022learning} utilizes Transformers to generate more integral initial pseudo labels for the end-to-end weakly-supervised semantic segmentation task and proposes an Affinity from Attention (AFA) module to learn semantic affinity from the multi-head self-attention (MHSA) in Transformers.
%Ru \textit{et al.} introduces the Transformers in weakly-supervised semantic segmentation (\textbf{WSSS}) to naturally incorporate the global information. 
Similar to \cite{ru2022learning}, we propose to integrate the Transformer architecture into our \textbf{UHR} image refinement segmentation task and leverage the learned semantic affinity from multi-head self-attention to enhance the precision of coarse masks. 



%-------------------------------------------------------------------------
\subsection{Hypernetworks}

Hypernetworks or meta-models, as referenced in \cite{article, littwin2019deep}, involve designing models specifically tailored for generating parameters for other models. This parameterization approach not only enhances the model's expressiveness, as highlighted in \cite{galanti2020comparing,galanti2020modularity}, but it also supports data compression through weight sharing across a meta-model \cite{article}. 
Unlike conventional deep neural networks, where the weights remain fixed during inference, hypernetworks possess the ability to generate adaptive weights or parameters for target networks \cite{li2022misf, guo2021jpgnet, Li_2023_ICCV, zhang2023superinpaint}. We leverage this technique and propose an Adaptive Implicit Representation Mapping Function. Essentially, an additional Convolution Network is responsible for learning the parameters of the implicit function in the segmentation network,
%Compared with the basic implicit function, our method with the newly acquired parameters incorporates global information features from the image, 
enhancing its adaptability to a variety of high-resolution image segmentation tasks. 
%In addition,  DNNs trained with hypernets can have fewer or similar weights than the corresponding standard DNNs, resulting in weight compression \cite{zhao2020meta}. Our lightweight network not only achieves parameter equivalency with the original MLP but also conditionally selects the adapted parameters depending on the variability of input images.


%-------------------------------------------------------------------------
